Net2Vec: Quantifying and Explaining how Concepts are Encoded by Filters in Deep Neural Networks

In an effort to understand the meaning of the intermediate representations captured by deep networks, recent papers have tried to associate specific semantic concepts to individual neural network filter responses, where interesting correlations are often found, largely by focusing on extremal filter responses. In this paper, we show that this approach can favor easy-to-interpret cases that are not necessarily representative of the average behavior of a representation. A more realistic but harder-to-study hypothesis is that semantic representations are distributed, and thus filters must be studied in conjunction. In order to investigate this idea while enabling systematic visualization and quantification of multiple filter responses, we introduce the Net2Vec framework, in which semantic concepts are mapped to vectorial embeddings based on corresponding filter responses. By studying such embeddings, we are able to show that 1., in most cases, multiple filters are required to code for a concept, that 2., often filters are not concept specific and help encode multiple concepts, and that 3., compared to single filter activations, filter embeddings are able to better characterize the meaning of a representation and its relationship to other concepts.

==> extra.tex <==
\pagebreak
\section{Extra}
\begin{itemize}
\item Main hypothesis:
\begin{itemize}
\item Looking at individual filters does not provide a full picture.
\item Visualizing the best examples from individual filters is misleading as it fails to note that this does not represent the full picture.
\end{itemize}

\item How we do it:
\begin{itemize}
\item We show that much better performance on BRODEN segmentation and ImageNet classification can be improved substantially by looking at combinations of filter responses.
\item We show that in particular images for which individual filters  respond very strongly may look good, but are not representative of the majority of images for which good results can be obtained from filter combinations.
\item This questions the view that individual filters capture specific concepts. Individual filters do respond more strongly that the vast majority of random filter combinations to certain concepts. Yet, specific filter combinations can be substantially better still.
\item For a given concept, we compare the best filter to the best linear combination of filters. We also rank filters by their weight in the combination and show two things. First, the filter that receives the largest weight is the one that is also the best individual predictor, as expected. Second, there are many other filters that have significant correlation with the concept. Third, only for some of the concept the best filter has a significantly stronger correlation than the others.
\item We also visualize ``saliency'' maps as the weighed sum of filter respones and show better results than using individual filters.
\item Note that in the Torralba's paper they have more concepts than filters, so what they do cannot be done properly.
\end{itemize}

\item Next, we look at concept embeddings. We treat each w vector as as a parametrization of the filter activations that correspond to a certain concept.
\begin{itemize}
\item We visualize then with t-SNE
\item We measure the alignment of the concept embedding learned using our method and a word embedding such as word2vec~\cite{X}. We compare that to the individual filers embedding.
\end{itemize}

\end{itemize}

%\begin{figure*}\centering
%\includegraphics[width=\linewidth]{viz_dist_relu5_comb_house_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_single_house_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_comb_dog_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_single_dog_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_comb_train_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_single_train_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_comb_plant_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_single_plant_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_comb_airplane_upsample_first.png}
%\includegraphics[width=\linewidth]{viz_dist_relu5_single_airplane_upsample_first.png}
%\caption{\textbf{Odd rows:} visualizations using learned segmentation weights. \textbf{Even rows:} visualizations using the best filter.}
%\label{f:viz_dist_upsample_first_extra}
%\end{figure*}

\begin{figure}
\centering
\includegraphics[width=0.49\linewidth]{viz_top_4_with_best_filter_house_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_linear_seg_house_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_best_filter_dog_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_linear_seg_dog_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_best_filter_plant_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_linear_seg_plant_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_best_filter_airplane_relu5.png}
\includegraphics[width=0.49\linewidth]{viz_top_4_with_linear_seg_airplane_relu5.png}
\label{f:viz_max_acts_single_extra}
\caption{Examples images that are maximally activated and aligned to the best relu5 filters (left) and to the learned weights (right) for the `house', `dog', `plant', and `airplane' concepts, for comparison with the non-maximal examples in~\cref{f:viz_dist} (those for the `train' filter were not coherent and are included in supplemental material) *For slightly smoother visualizations, activations were upsampled before being thresholded.}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.3\linewidth]{tsne_relu1_voc.png}
\includegraphics[width=0.3\linewidth]{tsne_relu2_voc.png}
\includegraphics[width=0.3\linewidth]{tsne_relu3_voc.png}

\includegraphics[width=0.3\linewidth]{tsne_relu4_voc.png}
\includegraphics[width=0.3\linewidth]{tsne_relu5_voc.png}
\end{center}
\caption{t-SNE visualizations of VOC Pascal concepts' learned weights.}
\label{f:tsne_extra}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\linewidth]{dist_set_ious_relu1.png}
\includegraphics[width=0.3\linewidth]{dist_set_ious_relu2.png}
\includegraphics[width=0.3\linewidth]{dist_set_ious_relu3.png}

\includegraphics[width=0.3\linewidth]{dist_set_ious_relu4.png}
\includegraphics[width=0.3\linewidth]{dist_set_ious_relu5.png}
\includegraphics[width=0.3\linewidth]{perc_combo_better_than_filter.png}
\end{center}
\caption{Distribution of Set IOUs by AlexNet layer.}
\label{f:dist_set_ious_extra}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\linewidth]{factor_of_improvement_relu1.png}
\includegraphics[width=0.3\linewidth]{factor_of_improvement_relu2.png}
\includegraphics[width=0.3\linewidth]{factor_of_improvement_relu3.png}

\includegraphics[width=0.3\linewidth]{factor_of_improvement_relu4.png}
\includegraphics[width=0.3\linewidth]{factor_of_improvement_relu5.png}
\end{center}
\caption{Factor of improvement graphs.}
\label{f:factor_of_improvement_extra}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\linewidth]{object_size_vs_class_size_relu1_all.png}
\includegraphics[width=0.3\linewidth]{object_size_vs_class_size_relu2_all.png}
\includegraphics[width=0.3\linewidth]{object_size_vs_class_size_relu3_all.png}

\includegraphics[width=0.3\linewidth]{object_size_vs_class_size_relu4_all.png}
\includegraphics[width=0.3\linewidth]{object_size_vs_class_size_relu5_all.png}
\end{center}
\caption{Object size vs. class size (explanation of the concepts for which best filter > combo).}
\label{f:object_size_versus_class_size_extra}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.49\linewidth]{dist_set_ious_relu5.png}
\includegraphics[width=0.49\linewidth]{object_size_vs_class_size_relu5_all.png}
\caption{\textbf{Left:} Distribution of Set IoU scores when using learned weights (blue) vs. the best filter (orange). \textbf{Right:} Concept dataset size plotted against mean concept, object size; this shows that failures occur (i.e., where a single filter outperforms our weighted, multi-filter approach) for concepts that are very small or have very few examples.}
\label{f:object_size_versus_class_size_main_extra}
\end{figure}

%\includegraphics[width=0.44\linewidth]{classification_accuracy_by_number_of_filters.png}


==> fig-beyond-top.tex <==
\begin{figure}[t]
\begin{center}
  %\includegraphics[width=\linewidth]{bau_fig_5.png}
\end{center}
\caption{~\cite{bau2017network}'s Fig. 5 shows the segmentation generated by each unit for the three Broden images with the highest activations.}
\label{f:beyond-top}
\end{figure}

==> method.tex <==
\section{Learning Net Embeddings}

%\begin{equation}
%AP_{k,c} = \frac{\sum_{i \in \mathcal{C}} IOU_{ind(i,k,c)}}{\sum_{i \in \mathcal{C}} \mathbb{I}[IOU_{ind(i,k,c)} > 0]}
%\end{equation}

\begin{enumerate}
\item ~\cite{bau2017network}'s method doesn't generalize well between different splits (i.e., choosing the best filter from training examples and then using that to evaluate on validation examples)
\end{enumerate}

\subsection{Theoretical Limit for a Perfectly Distributed Embedding Space}
Imagine a binary embedding space with $K$ dimensions; then, embeddings can be given by $x \in \{0,1\}^K$. Suppose that embeddings $x_1, x_2$ were constrained to be one-hot vectors; then, $||x_1|| = ||x_2|| = 1$,  $|x_1 \cdot x_2| = \{0,1\}$; thus, $\cos \theta = \frac{|x_1 \cdot x_2|}{||x_1|| ||x_2||} \in \{0,1\}$, where $\theta$ is the angle between $x_1$ and $x_2$. If embeddings $x_1, x_2$ were constrained to be ``two-hot'' vectors (i.e., they contain $1$s in two dimensions and $0$s elsewhere), then $||x_1|| = ||x_2|| = \sqrt{2}$, $|x_1 \cdot x_2| = \{0,1,2\}$, and $\cos \theta \in \{0,\frac{1}{2},1\}$.

In the general case, if embeddings $x_1, x_2$ were constrained to be $H$-hot vectors, where $H \in \{1,2,\ldots,\frac{K}{2}\}$, then $\cos \theta \in \{0, \frac{1}{H}, \ldots, \frac{H-1}{H}, 1\}$.  For embeddings constrained to be $H$-hot vectors, where $H \in \{\frac{K}{2},\frac{K}{2}+1, \ldots, K-1, K\}$, the minimum overlap is lower bounded by $|x_1 \cdot x_2| \geq K - 2(K - H)$; thus, $\cos \theta \in \{\frac{K - 2(K-H)}{H}, \ldots, \frac{H-1}{H}, 1 \}$. In both general cases, the smallest possible angle between any two $x_1, x_2$ $H$-hot embeddings, where $x_1, x_2$, is given by $\theta \geq \arccos(\frac{H-1}{H})$.

Now, suppose that $x_1$ was constrained to be a $H_1$-hot vector but $x_2$ could be any $H_2$-hot vector such that $H_2 < H_1$. The maximum amount of overlap between $x_1, x_2$ as given by the dot product is upper bounded by $|x_1 \cdot x_2| \leq H_2$; then, the smallest possible angle between $x_1$ and $x_2$ is given by $\theta \geq \arccos \frac{H_2}{\sqrt{H_1}\sqrt{H_2}} = \arccos \frac{\sqrt{H_2}}{\sqrt{H_1}}$.

(TODO: figure out edge case $\frac{K}{2}$ and odd/even cases, i.e., when $K$ is odd vs. even)


==> overview.tex <==
\section{Overview}\label{s:overview}

In this paper, we conduct a thorough analysis to investigate how semantic concepts, such as objects and their parts, are encoded by CNN filters. In particular, we consider two questions:
\begin{enumerate}
\item To what extend are individual filters sufficient to express a concept? Or, or are multiple filters required to code for a single concept?
\item To what extent does a filter exclusively code for a single concept? Or, is a filter shared by many, diverse concepts?
\end{enumerate}
While the answer to the above questions depends on the specific filter or concept under consideration, we demonstrate how to \textbf{quantify} the ``overlap'' of a filter or concept and show that there are many cases in which both notions of coverage do not hold. This means that, if we were to interpret semantic concepts and filter activations as corresponding set of images, in the resulting Venn's diagram the sets would intersect partially but neither kind of set would contain or be contained by the other.

While quantifying the relationship between concepts and representation may seem an obvious aim, so far much of the research on explaining how concepts are encoded by deep networks roughly falls into two more qualitative categories:
\begin{enumerate}
\item Interpretable visualizations of how single filters encode semantic concepts.
\item Demonstrations of distributive encoding with limited explanatory power of how a concept is encoded.
\end{enumerate}
In this work, we present methods that seek to marry the interpretive benefits of single filter visualizations with quantitative demonstrations of how concepts are encoded across multiple filters. We achieve this with our Net2Vec framework, which aligns semantic concepts with filter activations. It does so via concept embedding that learn how to weight filter activations to perform semantic tasks like segmentation and classification. Our concept vectors can be used to investigate both quantitatively \emph{and} qualitatively  the ``overlap'' of filters and concepts. Our novelty lies in outlining methods that go beyond simply demonstrating that multiple filters better encode concepts that single ones to quantifying and describing how a concept is encoded. Principally, we gain unique, interpretive power by formulating concepts vectors as embeddings.

As part of our analysis, we also highlight the problem with visualizing only the inputs that maximally activate a filter and propose evaluating the power of explanatory visualizations by how well they can explain the whole distribution of filter activations, not just the extreme ones.

\todo{Add links to other sections.}
